Hausa Visual Genome: A Dataset for Multi-Modal English to Hausa Machine Translation

Multi-modal Machine Translation (MMT) enables the use of visual information to enhance the quality of translations. The visual information can serve as a valuable piece of context information to decrease the ambiguity of input sentences. Despite the increasing popularity of such a technique, good and sizeable datasets are scarce, limiting the full extent of their potential. Hausa, a Chadic language, is a member of the Afro-Asiatic language family. It is estimated that about 100 to 150 million people speak the language, with more than 80 million indigenous speakers. This is more than any of the other Chadic languages. Despite a large number of speakers, the Hausa language is considered low-resource in natural language processing (NLP). This is due to the absence of sufficient resources to implement most NLP tasks. While some datasets exist, they are either scarce, machine-generated, or in the religious domain. Therefore, there is a need to create training and evaluation data for implementing machine learning tasks and bridging the research gap in the language. This work presents the Hausa Visual Genome (HaVG), a dataset that contains the description of an image or a section within the image in Hausa and its equivalent in English. To prepare the dataset, we started by translating the English description of the images in the Hindi Visual Genome (HVG) into Hausa automatically. Afterward, the synthetic Hausa data was carefully post-edited considering the respective images. The dataset comprises 32,923 images and their descriptions that are divided into training, development, test, and challenge test set. The Hausa Visual Genome is the first dataset of its kind and can be used for Hausa-English machine translation, multi-modal research, and image description, among various other natural language processing and generation tasks.

==> Makefile <==
LATEX=pdflatex
MAINFILE=main

default: $(MAINFILE).pdf

$(MAINFILE).pdf: lrec2022-example.bib

%.pdf: %.tex
	$(LATEX) $<
	bibtex $* || ( echo "Bibtex failed" && exit 1 )
	# change the exit 1 to exit 0 in the line above if you want to ignore it
	lim=4; \
	  while [ $$lim -ge 0 ] \
	      && grep 'Rerun to get\|Citation.*undefined' $*.log >/dev/null 2>/dev/null; do \
	    $(LATEX) $< ; \
	    lim=$$(($$lim - 1)) ; \
	  done

.PHONY: ci
ci:
	# make sure git will remember my password
	git config credential.helper store
	# git pull push dance with possibly uncommited local modifications
	if git pull --no-edit; then echo No changes to hide; else git stash; git pull --no-edit; git stash apply; fi; git commit -am "make ci by $(USER)"; git push

clean:
	rm -f $(MAINFILE).log $(MAINFILE).aux $(MAINFILE).bbl $(MAINFILE).blg $(MAINFILE).toc $(MAINFILE).out $(MAINFILE).run.xml $(MAINFILE).bcf


==> Result <==

Result files (output) are here:

https://drive.google.com/drive/folders/1Ry3bXzN3VuFYbobxLo-M7I10IRazaQjO

Text-to-Text Translation

Iteration 	&    Dev  &	    E-Test &	C-Test\\	
     5000	&    31.3 &    46.7   &	17.7	\\	    
     10000	&    29.9 &   47.2    &	17.0 \\	    
     15000	&    29.2 &   46.9    &	16.8 \\
     20000	&    29.2 &   46.3    &	16.8 \\
     25000	&    28.9 &   46.9    & 16.9   \\
     30000	&    29.0 &   46.7    & 17.0  \\
     35000	&    29.5 &   47.0    & 16.7  \\
     40000	&    29.2 &   47.2    & 16.4 \\
     45000  &    29.3 &   46.9    & 16.5  \\
     50000  &    29.1 &   47.1    & 16.8  \\
     55000  &    29.3 &   46.7    & 16.5  \\
     60000  &    29.4 &   46.5    & 16.5  \\
     65000  &    29.4 &   47.2    & 16.7 \\
     70000  &    30.0 &   46.6    & 16.6  \\
     75000  &    29.4 &   46.8    & 16.9  \\
     80000  &    29.8 &   46.7    & 16.2 \\
     85000  &    29.3 &   46.6    & 16.5  \\
     90000  &    28.9 &   46.7    & 16.3  \\
     95000  &    29.3 &   46.3    & 16.7  \\
     100000 &    29.6 &   46.3    & 16.4 \\


Multi-modal Translation-----------------------
Iteration 	&    Dev  &	    E-Test &	C-Test   \\	
     5000	&    16.2 &     23.6   &	8.4	      \\	    
     10000	&    16.1 &	    23.1   &    10.4       \\	    
     15000	&    15.2 &     21.3   &	10.3       \\
     20000	&    15.3 &     22.0   &	10.6         \\
     25000	&    14.8 &     23.3   &    10.3         \\
     30000	&    15.5 &     23.2   &   10.7            \\
     35000	&    13.4 &     20.5   &   10.0            \\
     40000	&    13.5 &     20.4   &   10.1            \\
     45000  &    13.1 &     19.9   &   9.9              \\
     50000  &    14.6 &     21.4   &   10.3                \\
     55000  &    14.0 &     20.3   &   10.1               \\
     60000  &    12.9 &     21.5   &   10.1       \\
     65000  &    13.1 &     20.4   &   10.0    \\
     70000  &    13.3 &     20.9   &   10.0    \\
     75000  &    13.2 &     19.9   &   9.3     \\
     80000  &    13.3 &     20.6   &   9.6     \\
     85000  &    12.6 &     18.9   &   9.1      \\
     90000  &    12.7 &     20.8   &   9.4     \\
     95000  &    13.0 &     20.0   &   9.6 \\
     100000 &    11.9 &     19.7   &   9.4\\

New Object Tag
----------------

Multi-modal Translation-----------------------
Iteration 	&    Dev  &	E-Test &	C-Test   \\	
     5000	&    15.7 & 22.6   &	8.2	      \\
     10000  &    15,1 & 20.8   &    6.7     \\
     15000  &          &        &             \\
     20000  &          &        &             \\
     25000  &         &          &            \\
     30000  &          &       &               \\
     35000  &         &         &              \\
     40000  &  13.6 & 20.0       & 6.1          \\


     

